LHC Phenomenology of the Three-Site Higgsless Model

We investigate the potential of the LHC for discovering the heavy vector and fermion resonances present in the Three-Site Higgsless Model. To this end, the model was implemented into the WHIZARD parton-level Monte Carlo eventgenerator. The results of parton-level simulations for different potential discovery channels are presented together with a discussion of the parameter space thus accessible at the LHC.

==> includes/app2.tex <==
\chapter{Useful Relations}

